Tosca: Operationalizing Commitments Over Information Protocols

The notion of commitment is widely studied as a high-level abstraction for modeling multiagent interaction. An important challenge is supporting flexible decentralized enactments of commitment specifications. In this paper, we combine recent advances on specifying commitments and information protocols. Specifically, we contribute Tosca, a technique for automatically synthesizing information protocols from commitment specifications. Our main result is that the synthesized protocols support commitment alignment, which is the idea that agents must make compatible inferences about their commitments despite decentralization.

==> Images/Interaction1.tex <==
\begin{tikzpicture}[>=stealth]

\draw[thick] (-2.5,1.4) node[above] {M} -- (-2.5,-1.1);
\draw[thick] (-0.9,1.4) node[above] {C}  -- (-0.9,-1.1);
\draw [thick](-1.7,1.4) node[above] {S} -- (-1.7,-1.1);

\node[cross out, draw=red, inner sep=0pt, outer sep=2pt] at (-0.9,1.2) {};
\draw[->, dashed, red] (-0.9,1.2) -- (-2.5,0.9)  node [midway, below, sloped] {\scriptsize{$\text{pay}_{\langle \text{oID1} \rangle}$}};


\node [left] at (-2.5,1.2) {\scriptsize{\textbf{M:cre(}$C^{P}$\textbf{)}}};
\draw[->] (-2.5,1.2) -- (-0.9,1) node [midway, above, sloped] {\scriptsize{$\text{quote}_{\langle \text{oID1} \rangle}$}};
\node [right] at (-0.9,1) {\scriptsize{{\textbf{C:cre(}$C^{P}$\textbf{)}}}};

\node[cross out, draw=red, inner sep=0pt, outer sep=2pt] at (-0.9,0.8) {};
\draw[->, dashed, red] (-0.9,0.8) -- (-2.5,0.5)  node [midway, below, sloped] {\scriptsize{$\text{pay}_{\langle \text{oID2} \rangle}$}};

\node [right] at (-0.9,0.4) {\scriptsize{{\textbf{C:det(}$C^{P}$\textbf{)}}}};
\draw[->] (-0.9,0.4) -- (-2.5,0.2)  node [midway, below, sloped] {\scriptsize{$\text{pay}_{\langle \text{oID1} \rangle}$}};
\node [left] at (-2.5,0.2) {\scriptsize{\textbf{M:det(}$C^{P}$\textbf{)}}};

\draw[->] (-2.5,-0.1) -- (-1.7,-0.2)node [midway, below, sloped] {\scriptsize{$\text{requestShip}_{\langle \text{oID1} \rangle}$}};

\draw[->](-1.7,-0.7) -- (-0.9,-0.8)node [midway, below, sloped] {\scriptsize{$\text{ship}_{\langle \text{oID1} \rangle}$}};
\node [right] at (-0.9,-0.8) {\scriptsize{{\textbf{C:dis(}$C^{P}$\textbf{)}}}};

\node at (-1.7,-1.5) {\scriptsize{(A)}};

\draw[thick] (1.7,1.4) node[above] {M} -- (1.7,-1.1);
\draw[thick] (3.5,1.4) node[above] {C}  -- (3.5,-1.1);
\draw[thick](2.3,1.4) node[above] {S} -- (2.3,-1.1);
\draw[thick] (2.9,1.4) node[above] {E}  -- (2.9,-1.1);


\node [left] at (1.7,1) {\scriptsize{\textbf{M:cre(}$C^{EP}$\textbf{)}}};
\draw[->] (1.7,1.3) -- (3.5,1.2) node [midway, below, sloped] {\scriptsize{$\text{quote}_{\langle \text{oID2} \rangle}$}};
\node [right] at (3.5,1.2) {\scriptsize{{\textbf{C:cre(}$C^{EP}$\textbf{)}}}};

\node [right] at (3.5,0.7) {\scriptsize{{\textbf{C:det(}$C^{EP}$\textbf{)}}}};
\draw[->] (3.5,0.7) -- (2.9,0.6)  node [midway, below, sloped] {\scriptsize{$\text{payEscrow}_{\langle \text{oID2} \rangle}$}};
\node [left] at (1.7,0.1) {\scriptsize{\textbf{M:det(}$C^{EP}$\textbf{)}}};
\draw[->] (3.5,0.2) -- (1.7,0.1)  node [midway, below, sloped] {\scriptsize{$\text{fwdCMPayEscrow}_{\langle \text{oID2} \rangle}$}};
\draw[->](1.7,-0.3) -- (2.3,-0.4)node [midway, below, sloped] {\scriptsize{$\text{requestShip}_{\langle \text{oID2} \rangle}$}};
\node [right] at (3.5,-1) {\scriptsize{{\textbf{C:dis(}$C^{EP}$\textbf{)}}}};
\draw[->](2.3,-0.9) -- (3.5,-1)node [midway, below, sloped] {\scriptsize{$\text{ship}_{\langle \text{oID2} \rangle}$}};
\node at (2.6,-1.5) {\scriptsize{(B)}};

\draw[thick] (-1.7,-2.3) node[above] {M} -- (-1.7,-6.2);
\draw[thick] (1.2,-2.3) node[above] {C}  -- (1.2,-6.2);
\draw [thick](-0.2,-2.3) node[above] {S} -- (-0.2,-6.2);
\draw[thick] (2.7,-2.3) node[above] {E}  -- (2.7,-6.2);
\node [left] at (-1.7,-2.4) {\scriptsize{\textbf{M:cre(}$C^{EP}$\textbf{)}}};
\draw[->] (-1.7,-2.4) -- (1.2,-2.5) node [midway, below, sloped] {\scriptsize{$\text{quote}_{\langle \text{oID3} \rangle}$}};

\draw[->] (-1.7,-2.8) -- (2.7,-3) node [midway, below, sloped] {\scriptsize{$\text{fwdMEQuote}_{\langle \text{oID3} \rangle}$}};
\node [right] at (2.7,-3) {\scriptsize{{\textbf{E:cre(}$C^{EP}$\textbf{)}}}};

\draw[->] (1.2,-3.6) -- (2.7,-4.1)  node [midway, below, sloped] {\scriptsize{\; \;\;\;\;\;\;\;\;$\text{payEscrow}_{\langle \text{oID3} \rangle}$}};
\node [right, text width = 3cm] at (2.7,-4.1) {\scriptsize{{\textbf{E:det(}$C^{EP}$\textbf{)}}} \\
{\textbf{E:cre(}$C^{EMP}$\textbf{)}}};
\node [left, text width = 1.5 cm] at (-1.7,-3.5) {\scriptsize{\textbf{M:det(}$C^{EP}$\textbf{)}} \\
\scriptsize{\textbf{M:cre(}$C^{EMP}$\textbf{)}}};
\draw[->] (1.2,-3.4) -- (-1.7,-3.5)  node [midway, below, sloped] {\scriptsize{$\text{fwdCMPayEscrow}_{\langle \text{oID3} \rangle}$}};
\draw[->](-1.7,-3.9) -- (-0.2,-4.1)node [midway, below, sloped] {\scriptsize{$\text{requestShip}_{\langle \text{oID3} \rangle}$}};
\draw[->](-0.2,-4.5) -- (1.2,-4.6)node [midway, below, sloped] {\scriptsize{$\text{ship}_{\langle \text{oID3} \rangle}$}};
\draw[->](-0.2,-4.7) -- (-1.7,-5.1)node [midway, below, sloped] {\scriptsize{$\text{fwdSMShip}_{\langle \text{oID3} \rangle}$}};
\node [left, text width = 1.7 cm] at (-1.7,-5.1) {\scriptsize{\textbf{M:dis(}$C^{EP}$\textbf{)}} $\rightarrow$ \\
\scriptsize{\textbf{M:det(}$C^{EMP}$\textbf{)}}};
\draw[->](-0.2,-5.1) -- (2.7,-5.2)node [midway, below, sloped] {\scriptsize{$\text{fwdSEShip}_{\langle \text{oID3} \rangle}$}};
\node [right, text width = 3cm] at (2.7,-5.2) {\scriptsize{{\textbf{E:dis(}$C^{EP}$\textbf{)}}} $\rightarrow$ \\ \textbf{E:det(}$C^{EMP}$\textbf{)}};
\node [right] at (2.7,-5.9) {\scriptsize{{\textbf{E:dis(}$C^{EMP}$\textbf{)}}}};
\draw[->](2.7,-5.9) -- (-1.7,-5.9)node [midway, below, sloped] {\scriptsize{$\text{transfer}_{\langle \text{oID3} \rangle}$}};
\node [left] at (-1.7,-5.9) {\scriptsize{{\textbf{M:dis(}$C^{EMP}$\textbf{)}}}};

\node at (0.4,-6.5) {\scriptsize{(C)}};

\end{tikzpicture}

==> Images/Interaction2.tex <==
\begin{tikzpicture}[>=stealth]
\setlength{\fboxsep}{1pt}

\draw[thick] (-2.5,1.4) node[above] {M} -- (-2.5,-1.1);
\draw[thick] (-0.3,1.4) node[above] {C}  -- (-0.3,-1.1);
\draw [thick](-1.4,1.4) node[above] {S} -- (-1.4,-1.1);



\draw[->] (-2.5,1.2) -- (-0.3,0.7) node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{quote}$}}};
\draw[thick, dashed, blue] (-2.9,1) node[left]{1} -- (0.1,0.9);
\draw[->] (-0.3,0.6) -- (-2.5,0.3)  node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{pay}$}}};
\draw[thick, dashed, blue] (-2.9,0.4) node[left]{2} -- (0.1,0.4);
\draw[->] (-2.5,-0.1) -- (-1.4,-0.2)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{requestShip}$}}};
\draw[thick, dashed, blue] (-2.9,0) node[left]{3} -- (0.1,0);
\draw[->](-1.4,-0.7) -- (-0.3,-0.8)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{ship}$}}};
\draw[thick, dashed, blue] (-2.9,-0.9) node[left]{4} -- (0.1,-0.9);
\node at (-1.4,-1.5) {\scriptsize{A}};

\draw[thick] (1.1,1.4) node[above] {M} -- (1.1,-1.1);
\draw[thick] (3.5,1.4) node[above] {C}  -- (3.5,-1.1);
\draw[thick](1.9,1.4) node[above] {S} -- (1.9,-1.1);
\draw[thick] (2.7,1.4) node[above] {E}  -- (2.7,-1.1);

\draw[->] (1.1,1.3) -- (3.5,1.2) node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{quote}$}}};
\draw[->] (3.5,1.1) -- (2.7,1)  node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{payEscrow}$}}};
\draw[thick, dashed, blue] (0.7,0.5) node[left]{5} -- (3.9,0.5);
\draw[->] (3.5,0.3) -- (1.1,0.1)  node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{fwdCMPayEscrow}$}}};
\draw[thick, dashed, blue] (0.7,-0.3) node[left]{6} -- (3.9,-0.3);
\draw[->](1.1,-0.5) -- (1.9,-0.6)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{requestShip}$}}};
\draw[->](1.9,-1) -- (3.5,-1.1)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{ship}$}}};
\node at (2.1,-1.5) {\scriptsize{B}};

\draw[thick] (-1.7,-2.3) node[above] {M} -- (-1.7,-6.2);
\draw[thick] (1.2,-2.3) node[above] {C}  -- (1.2,-6.2);
\draw [thick](-0.2,-2.3) node[above] {S} -- (-0.2,-6.2);
\draw[thick] (2.7,-2.3) node[above] {E}  -- (2.7,-6.2);

\draw[->] (-1.7,-2.4) -- (1.2,-2.5) node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{quote}$}}};

\draw[->] (-1.7,-2.8) -- (2.7,-3) node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{fwdMEQuote}$}}};

\draw[->] (1.2,-3.6) -- (2.7,-3.8)  node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{payEscrow}$}}};

\draw[->] (1.2,-3.4) -- (-1.7,-3.5)  node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{fwdCMPayEscrow}$}}};
\draw[->](-1.7,-3.8) -- (-0.2,-4.1)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{requestShip}$}}};
\draw[->](-0.2,-4.3) -- (1.2,-4.4)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{ship}$}}};
\draw[->](-0.2,-4.5) -- (-1.7,-4.7)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{fwdSMShip}$}}};
\draw[thick, dashed, blue] (-2.1,-5.1) node[left]{7} -- (3.1,-5.1);
\draw[->](-0.2,-5.2) -- (2.7,-5.3)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{fwdSEShip}$}}};
\draw[thick, dashed, blue] (-2.1,-5.7) node[left]{8} -- (3.1,-5.7);

\draw[->](2.7,-5.9) -- (-1.7,-6.1)node [midway, below, sloped] {\scriptsize{\colorbox{white}{$\text{transfer}$}}};

\node at (0.4,-6.5) {\scriptsize{C}};

\end{tikzpicture}
